Traffic-CBM: A Structurally Interpretable Multimodal Framework for Encrypted Traffic Classification

Encrypted traffic classification has achieved strong performance, but its decision process remains difficult to interpret. Existing methods usually combine flow statistics, packet sequences, and byte-level representations into opaque latent features, making it unclear which type of evidence actually drives the prediction. In this paper, we propose Traffic-CBM, a structurally interpretable multimodal framework for encrypted traffic classification. Instead of directly fusing heterogeneous traffic signals into a black-box representation, Traffic-CBM organizes them into a unified hierarchical concept space. These concepts are not manually annotated semantic attributes; rather, they are scalar evidence summaries constrained by predefined traffic evidence groups. More specifically, grouped flow statistics are mapped to statistical concepts, dedicated temporal encoders learn temporal concepts from disjoint feature subspaces, and byte-level evidence is further organized into packet-level and cross-packet concepts. This design turns heterogeneous traffic evidence into an explicit concept representation and makes different levels of traffic evidence easier to analyze. We evaluate Traffic-CBM on multiple encrypted traffic benchmarks. Results show that it achieves competitive and balanced classification performance while providing a clearer structural interpretation interface than conventional end-to-end fusion models. Further analyses suggest that the learned concept space is actively used in the prediction process and provides a clearer structural explanation of multimodal traffic evidence.

==> tabs/complexity.tex <==
\begin{table}[t]
\centering
\caption{Complexity comparison with existing methods. 
Parameter counts follow the settings reported in the original papers, 
where classification heads are not included and only backbone parameters are considered.}
\label{tab:complexity}
\setlength\tabcolsep{5pt}
\small
\begin{tabular}{lcccc}
\toprule
Model 
& Params(M) 
& FLOPs(G) 
& Mem(MB) 
& Time(ms) \\
\midrule
AppScanner              & -     & 0.0   & 0.0   & 0.0 \\
DeepFP                  & 2.4   & 0.0   & 0.0   & 0.0 \\
FS-Net                  & 2.9   & 0.0   & 0.0   & 0.0 \\
ET-BERT                 & 132.2 & 0.0   & 0.0   & 0.0 \\
NetMamba                & 1.9   & 0.0   & 0.0   & 0.0 \\
YaTC                    & 1.9   & 0.0   & 0.0   & 0.0 \\
TrafficFormer           & 132.2 & 0.0   & 0.0   & 0.0 \\
\textbf{Traffic-CBM}    & 5.2   & 0.0   & 0.0   & 0.0 \\
\bottomrule
\end{tabular}
\end{table}

==> tabs/drift.tex <==
\begin{table*}[t]
\centering
\caption{Results on CipherSpectrum(AES128), CipherSpectrum(Mix), and (CSTNET-TLS13).}
\label{tab:results_part1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccc|cccc|cccc}
\toprule

Datasets
& \multicolumn{4}{c|}{CipherSpectrum(AES128)}
& \multicolumn{4}{c|}{CipherSpectrum(Mix)}
& \multicolumn{4}{c}{CSTNET-TLS13} \\

\midrule

Approaches
& AC & PR & RC & F1
& AC & PR & RC & F1
& AC & PR & RC & F1 \\

\midrule

ET-BERT
& 0.4512 & 0.4575 & 0.4512 & 0.3898
& 0.3280 & 0.3565 & 0.3280 & 0.2781
& 0.4610 & 0.4220 & 0.3992 & 0.3691 \\

YaTC
& - & - & - & -
& - & - & - & -
& - & - & - & - \\

TrafficFormer
& 0.4159 & 0.3978 & 0.4159 & 0.3911
& 0.3249 & 0.3477 & 0.3249 & 0.2786
& 0.6592 & 0.6367 & 0.6194 & 0.6141 \\

NetMamba
& 0.4078 & 0.3582 & 0.4080 & 0.3435
& 0.3437 & 0.3029 & 0.3437 & 0.2859
& 0.8947 & 0.8980 & 0.8944 & 0.8926 \\

\midrule

Traffic-CBM
& - & - & - & -
& - & - & - & -
& - & - & - & - \\

\quad 6+1+1
& 0.8998 & 0.9040 & 0.8998 & 0.8994
& - & - & - & -
& 0.5918 & 0.5447 & 0.5347 & 0.5231 \\

\quad 6/6/6
& 0.9588 & 0.9613 & 0.9588 & 0.9589
& - & - & - & -
& 0.6831 & 0.6513 & 0.6256 & 0.6188 \\

\quad 6+4|b
& 0.9361 & 0.9395 & 0.9361 & 0.9362
& - & - & - & -
& 0.6967 & 0.6756 & 0.6568 & 0.6542 \\

\quad 6+4+5+3
& 0.9407 & 0.9424 & 0.9407 & 0.9406
& 0.9329 & 0.9354 & 0.9329 & 0.9331
& 0.7514 & 0.7417 & 0.7154 & 0.7139 \\

\bottomrule
\end{tabular}
}
\end{table*}


\begin{table*}[t]
\centering
\caption{Results on ISCX-VPN(App), ISCX-VPN(Service), and USTC-TFC2016.}
\label{tab:results_part2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cccc|cccc|cccc}
\toprule

Datasets
& \multicolumn{4}{c|}{ISCX-VPN(App)}
& \multicolumn{4}{c|}{ISCX-VPN(Service)}
& \multicolumn{4}{c}{USTC-TFC2016} \\

\midrule

Approaches
& AC & PR & RC & F1
& AC & PR & RC & F1
& AC & PR & RC & F1 \\

\midrule

ET-BERT
& 0.6532 & 0.5523 & 0.5505 & 0.5341
& 0.7237 & 0.5787 & 0.6248 & 0.5985
& 0.9872 & 0.9889 & 0.9843 & 0.9865 \\

YaTC
& - & - & - & -
& - & - & - & -
& - & - & - & - \\

TrafficFormer
& 0.7162 & 0.6587 & 0.6693 & 0.6543
& 0.7763 & 0.7395 & 0.7601 & 0.7420
& 0.9872 & 0.9883 & 0.9852 & 0.9867 \\

NetMamba
& 0.8000 & 0.7891 & 0.8000 & 0.7877
& 0.8996 & 0.9032 & 0.8996 & 0.9004
& 0.9910 & 0.9910 & 0.9910 & 0.9909 \\

\midrule

Traffic-CBM
& - & - & - & -
& - & - & - & -
& - & - & - & - \\

\quad 6+1+1
& 0.6622 & 0.5416 & 0.5275 & 0.5163
& - & - & - & -
& - & - & - & - \\

\quad 6/6/6
& 0.7883 & 0.7364 & 0.7206 & 0.7251
& - & - & - & -
& 0.9904 & 0.9915 & 0.9879 & 0.9896 \\

\quad 6+4|b
& 0.7117 & 0.5706 & 0.5908 & 0.5727
& 0.8553 & 0.8680 & 0.8288 & 0.8330
& 0.9895 & 0.9922 & 0.9848 & 0.9882 \\

\quad 6+4+5+3
& 0.7838 & 0.7083 & 0.6894 & 0.6925
& 0.8991 & 0.8970 & 0.8800 & 0.8843
& 0.9914 & 0.9924 & 0.9898 & 0.9911 \\

\bottomrule
\end{tabular}
}
\end{table*}
